Double parton scattering singularities in two-loop gluon-fusion amplitudes

Gluon fusion to two massive colour singlets can develop a double parton scattering (DPS) singularity as $p_T\to0$: each gluon splits, and its daughters fuse pairwise. We determine two-loop logarithms using a common kernel and derive finite matching functions analytically for gluon and quark splittings. Normalised to one loop, the cubic coefficient changes sign between channels. Complete $gg\to HH$, $gg\to AA$ and $gg\to ZZ$ amplitudes confirm the predicted colour, helicity and parity dependence and phase. The kernel gives leading DPS logarithms for other pairs with this DPS configuration.

==> letter_labels.tex <==
% generated by letter_labels.py from letter.aux; do not edit
\LetterLabel{eq:Fm}{11}
\LetterLabel{eq:factorised}{1}
\LetterLabel{eq:gammaK}{2}
\LetterLabel{eq:imK}{6}
\LetterLabel{eq:kernel}{3}
\LetterLabel{eq:n4exp}{9}
\LetterLabel{eq:oneloop}{5}
\LetterLabel{eq:r0g}{7}
\LetterLabel{eq:r0q}{8}
\LetterLabel{eq:rapcoef}{12}
\LetterLabel{eq:rg}{4}
\LetterLabel{eq:threeloop}{10}
\LetterLabel{fig:dps}{1}
\LetterLabel{tab:n4letter}{II}
\LetterLabel{tab:threeloop}{III}

